What's the Meaning of Superhuman Performance in Today's NLU?

In the last five years, there has been a significant focus in Natural Language Processing (NLP) on developing larger Pretrained Language Models (PLMs) and introducing benchmarks such as SuperGLUE and SQuAD to measure their abilities in language understanding, reasoning, and reading comprehension. These PLMs have achieved impressive results on these benchmarks, even surpassing human performance in some cases. This has led to claims of superhuman capabilities and the provocative idea that certain tasks have been solved. In this position paper, we take a critical look at these claims and ask whether PLMs truly have superhuman abilities and what the current benchmarks are really evaluating. We show that these benchmarks have serious limitations affecting the comparison between humans and PLMs and provide recommendations for fairer and more transparent benchmarks.

==> explanations-old.tex <==
\section{Explanations in NLP}
\label{sec:explanations-old}
%TD I am wondering if looking at on how explanations look like when observing human performances in a tasks. My first feeling is that we are looking at explanations when humans are failing, but less when they are giving a correct response. Checking this.
An important shortcoming of current NLP systems is their limited ability to explain predictions in a faithful way. This is problematic for at least three reasons. First, as NLP researchers, it is important to understand why predictions are made to make sure that models are right for the right reasons \cite{mccoy-etal-2019-right,niven-kao-2019-probing}, or to uncover some of the shortcuts that the model may have learned \cite{geirhos2020shortcut}. More generally, explanations can help us to better understand what it would take to achieve a step change in performance, e.g.\ to find out whether the model is failing because it lacks access to particular world knowledge, because it fails to reason about the information provided in a correct way, or because of something else. Second, explainability is important for regulators and the general public to assess whether, or in what contexts, a system is safe to use. For instance, explanations can help us to uncover unwanted biases in the system, or the fact that it relies on outdated knowledge. Note that in this case, explanations are used to gain an understanding of the system's behavior as a whole. Third, explanations are useful for end users, to help them judge when they can trust a given prediction.

The absence of explanations of performance easily lead researchers astray. For example, the prize-winning paper by Kaushik and Lipton \cite{emnlp-2018-kaushik-lipton} shows how several state of the art QA systems that purport to read paragraphs and answer multiple-choice questions about them do almost as well, on a variety of datasets, when either the paragraphs or the questions are masked or withheld and just the candidate answers are presented. Language-model based QA systems simply classify the best matching answer to (respectively) either the question or the paragraph, using their pre-stored knowledge about each question candidate, without performing any `reading' or actual QA. None of the authors of the QA systems used in this study had considered this possibility, or had thought to require explanations from their QA systems. 

\subsection{What should explanations look like?}
While the desirability of high-quality explanations is rather uncontroversial, it is less clear what form such explanations should take. For tasks such as sentiment classification, it may be sufficient to highlight which words from the input text have mostly affected a given prediction. Consider, however, the problem of closed-book question answering and a question such as ``What is the capital of Italy?''. What should an explanation for the predicted answer look like? In this case, the main purpose of the explanation is to allow us to assess whether we can trust the answer. A system that can produce well-calibrated confidence estimates would thus largely eliminate the need for explanations. Unfortunately, it is not clear whether confidence estimates that are faithful at the level of individual predictions can realistically be obtained. Moreover, for many settings, we may still need explanations to justify why the system puts a high confidence in a particular answer (e.g.\ to understand why the system confidently predicts an incorrect answer). 

For Natural Language Inference (NLI) and question answering (QA), several datasets with explanations have recently been introduced \cite{camburu2018snli,rajani-etal-2019-explain,aggarwal-etal-2021-explanations}. In these cases, explanations take the form of natural language sentences, which aim to clarify why the hypothesis is (or is not) entailed or contradicted by a given premise. Consider, for instance, the following example from e-SNLI \cite{camburu2018snli}:

\medskip
\noindent \textsc{Premise}: \emph{Children smiling and waving at camera}\\
\noindent \textsc{Hypothesis}: \emph{They are smiling at their parents}\\
\noindent \textsc{Explanation}: \emph{Just because they are smiling and waving at a camera does not imply their parents or anyone is anyone behind it}
\medskip

\noindent Essentially, this explanation paraphrases the assertion that the hypothesis is not entailed by the premise, without providing any real insights. NLP systems can be trained to generate such human-generated explanations, but it is unclear whether this can help us to better understand why and when systems are making mistakes (although training the model on explanations can in some cases benefit overall model performance). In fact, \citet{camburu-etal-2020-make} highlighted the fact that models can generate contradictory explanations for the same input, e.g.\ at the same time arguing that a hypothesis is entailed because ``snowboarding is done outside'' and arguing that it is not because ``snowboarding is not done outside''. Such findings cast doubts on the usefulness of generated explanations for understanding how the model behaves.

\subsection{Towards faithful explanations}
Given the aforementioned considerations, in many cases, providing explanations that are reflective of the behavior of the model only seems possible by moving away from the standard paradigm of prompting or fine-tuning language models. We now discuss in more detail what would be required for generating faithful explanations in NLI or QA settings. Fundamentally, an explainable system needs to be explicit about what it believes to be true, and how different beliefs can be combined to infer further beliefs. Such a system would need to have the following abilities:
\begin{itemize}
\item We need a \emph{fact extraction} mechanism to find out what the system believes to be true. This could be achieved, for instance, by generating knowledge graph triples from a language model that is fine-tuned for that purpose, as e.g.\ in the case of COMET \cite{bosselut-etal-2019-comet}. 
\item We need a task-agnostic mechanism to infer novel facts from a given set of premises. Here, it is crucial that this \emph{inference model} is operating without access to what we are trying to prove or disprove, to ensure that inferences reflect the beliefs of the system, rather than being driven by the need to generate a particular post-hoc explanation.
\item Finally, we need a mechanism to solve the actual task, using the inference model to combine information provided in the input (i.e.\ premise and hypothesis) with knowledge obtained by the fact extraction mechanism.
\end{itemize}
These three elements are present in some form in the approach proposed by \citet{tafjord2022entailer}, where a QA system is trained on a set of manually constructed entailment trees. The leaves of these trees can be viewed as atomic facts, which are combined into increasingly more complex statements, until the given answer candidate can be proved. We believe this approach to be an important step in the right direction, although several significant challenges remain. First, while the approach was presented as a general purpose reasoning system, it was trained on a relatively small collection of 1840 science questions. Given the cost involved in obtaining large sets of high-quality entailment trees, scaling up this approach based on direct supervision is not realistic. Second, the approach crucially relies on standard deductive reasoning, which is not sufficient in many contexts. For instance, we may need to reason with defeasible knowledge to arrive at a given answer, or rely on aggregating pieces of evidences that may individually be quite weak.

Another line of relevant work relies on chain-of-thought prompting \cite{wei2022chain}, i.e.\ the finding that large language models can generate inference chains based on a small number of examples of such chains. This was found to improve the ability of such models to answer questions that require reasoning, while the inference chains themselves could serve as explanations. However, even when the inference chains are semantically valid, there are no guarantees that they accurately reflect the inference process that was used by the model, i.e.\ the explanations are not necessarily faithful, in the terminology of \citet{tafjord2022entailer}. Moreover, this approach is again limited to cases where the result can be inferred in a straightforward way using a relatively small number of deductive steps.

==> reannotation-of-data.tex <==
\section{A Reannotation of Data}

We propose an experiment in which we reannotate a sample of data in a redundant way (i.e., 10 annotators?) on a sample of x\% of data items. Objectives:

\begin{itemize}
    \item Determine who is the "best" human annotator (to compare against the "best" machine): is it the best performing annotator? does majority voting help solve all the issues? let's ask annotators to tag items as ambiguous or with missing context, so as to see whether this has impact on the resulting annotation.
    \item Determine who is the "worst" human annotator (thus, the performance range between good and bad annotators).
    \item Difference between boolean and complex tasks.
\end{itemize}

==> related-work.tex <==
\section{Related Work}

%What works talk about these issues?

